High performance reduction technique for multiscale finite element modeling (HPR-FE2): towards industrial multiscale FE software

The authors have shown in previous contributions that reduced order modeling with optimal cubature applied to finite element square (FE2) techniques results in a reliable and affordable multiscale approach, the HPR-FE2 technique. Such technique is assessed here for an industrial case study of a generic 3D reinforced composite whose microstructure is represented by two general microcells accounting for different deformation mechanisms, microstrucural phases and geometry arrangement. Specifically, in this approach the microstrain modes used for building the reduced order model (ROM) are obtained through standard proper orthogonal decomposition (POD) techniques applied over snapshots of a representative sampling strain space. Additionally, a reduced number of integration points is obtained by exactly integrating the main free energy modes resulting from the sampling energy snapshots. The outcome consists of a number of dominant strain modes integrated over a remarkably reduced number of integration points which provide the support to evaluate the constitutive behavior of the microstructural phases. It is emphasized that stresses are computed according to the selected constitutive law at the reduced integration points and, therefore, the strategy inherits advantageous properties such as model completeness and customization of material properties. Overall results are discussed in terms of the consistency of the multiscale analysis, customization of the microscopic material parameters and speedup ratios compared to high-fidelity finite element (HF) simulations.

==> section_results.tex <==
% !TeX spellcheck = en_GB
\section{HR-FE2 model assessment}
%
%
\textcolor{red}{Completar descripcion cuando la seccion este lista.}
The $\text{HR-FE}^2$ model is evaluated by simulating two typical layered-type composite microstructures undergoing a non-linear damage regime (\ref{sect_models})
In subsection \ref{sect_response}, we evaluate the error introduced by recovering the  reduced fields of the mechanical problem.
This recovery consists on projecting the solution fields onto the original finite element mesh.
In subsection \ref{sect_dogbone}, and adopting a second type of composite microstructure, we analyse a full multiscale problem.
The structure at the macroscopic level is a specimen subjected to a system of shear loads... In next subsection \ref{sect_speedup}, the order of  computational speedups attained with the $\text{HR-FE}^2$ model is analysed.
Typically, the more complex the micromodel is, the larger the speedup attained...
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Microscopic models}
\label{sect_models}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
The two models were considered in this work resemble fibre-reinforced composite laminate (\emph{composites}) with glass fibres and epoxy matrix.
%
The scope of this, however, is not necessarily the precise modelling of composites, but the demonstration of the technical capabilities of the HR-FE2 method and its correct representation of the failure modes of the damage model used.


The first RVE model "A" (see geometry and material values in figure~\ref{fig_regions_ref} and table~\ref{table_material_params_ref}) is a synthetic case aiming to manifest the main failure mechanisms in composites, including delamination of layers and pull-out between fibres and matrix. Bidirectional fibres.  Bidirectional composite lamina.
%
%
\begin{figure}[hbt]
    \centering
    \includegraphics[width=.5\textwidth]{figures_results/regions_ref_1}
    \qquad
    \includegraphics[width=.115\textwidth]{figures_results/regions_ref_0}
    \qquad
    \includegraphics[width=.12\textwidth]{figures_results/regions_ref_2}
    \caption{Regions of RVE "A" (from left to right): matrix, inclusion, cohesive, interply. Failure mechanisms modelled: damaged matrix regions, delamination between layers, and fiber pull-out and debonding between fiber and matrix.}
    \label{fig_regions_ref}
\end{figure}
%
\begin{table}[hbt]
    \centering
    \begin{tabular}{lcccc}
        \toprule
        & Matrix     & Inclusion   & Cohesive    & Interply    \\
        \midrule
        Young modulus $E$ [\si{N/mm^2}] & \num{3790} & \num{72000} & \num{3790}  & \num{3790}  \\
        Poisson ratio $\nu$& \num{0.37} & \num{0.25}  & \num{0.37}  & \num{0.37}  \\
        Elastic threshold $\sigma_{\text{e}}$ [\si{N/mm^2}] & \num{200}  & \num{20000} & \num{100}   & \num{100}   \\
        Infinity elastic threshold $\sigma_{\text{e}}$ [\si{N/mm^2}] & \num{220}  & \num{20001} & \num{100.1} & \num{100.1} \\
        Hardening parameter $H_1$& \num{0.10} & \num{0.10}  & \num{0.01}  & \num{0.01}  \\
        Hardening parameter $H_2$& \num{0.01} &     \num{0.10} &  \num{0.01} & \num{0.01}  \\
        \bottomrule
    \end{tabular}
    \caption{Material parameters of RVE regions.}
    \label{table_material_params_ref}
\end{table}


The second RVE model "B" aims to represent a more realistic geometry of unidirectional fibre-reinforced composite laminates.
%
Fibres are randomly distributed and a volume fraction of \SI{60}{\percent} (see figure~\ref{fig:regions_porto} and table~\ref{tab:material_params_porto} ).
%
This model, in contrast to RVE "A", does not have an interphase region to represent fibre pull-out, neither ply delamination.
%
%
\begin{figure}[hbt]
    \centering
    \includegraphics[width=.3\textwidth]{figures_results/regions_porto_0}
    \includegraphics[width=.3\textwidth]{figures_results/regions_porto_1}
    \includegraphics[width=.3\textwidth]{figures_results/regions_porto_2}
    \caption{Regions of RVE: matrix (left), inclusion (right) }
    \label{fig:regions_porto}
 \end{figure}
%
\begin{table}
    \centering
    \begin{tabular}{lcc}
        \toprule
        \Trule \Brule  & Matrix     & Inclusion    \\
        \midrule
        Young modulus $E$ [\si{N/mm^2}]                                        & \num{4000} & \num{231000} \\
        Poisson ratio $\nu$                                                                      & \num{0.38}  & \num{0.2}  \\
        Elastic threshold $\sigma_{\text{e}}$ [\si{N/mm^2}]       & \num{60}  & \num{1.0e8}\\
        Infinity elastic threshold $\sigma_{\text{e}}$ [\si{N/mm^2}] & \num{70}  & \num{1.1e8} \\
        Hardening parameter $H_1$                                                    & \num{0.335}  & \num{0.01} \\
        Hardening parameter $H_2$                                                    & \num{0.05}  &  \num{0.01} \\
        \bottomrule
    \end{tabular}
    \caption{Material parameters of RVE regions.}
    \label{tab:material_params_porto}
\end{table}


In both cases, RVE are periodic, fibres are assumed to behave elastically in the range od strain considered in this study, and matrices (and interphase in case of model A) are modelled by a traction-only damage model with linear hardening parameters $H_1$ and $H_2$ (see REFERENCE TO APENDIX)
%
\FloatBarrier
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Training }
\label{sect_training}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
In the training stage the high fidelity computation of the RVE under different strain states is computed.
%
High fidelity models have been implemented in KratosMultiphysics [REFERENCE].
Periodic boundary conditions.
AMGCL solver \cite{}
%
the parameter space contains any load path associated to the macro-strain over a certain period. Each trajectory is a monotonically growing load strain, fixed load increment for the timesteps.
Load: We calibrated the strain steps with a load factor $\mu$. Strain is applied to all integration points of the RVE.
We adjust the strain factor so most of the trajectories have entered the non-linear region (DESCRIBIR HASTA CUANDO)


The only difference between cases is the strain value, which eis the parameter of the training.
%
The training dataset is composed by 100 strain trajectories uniformly distributed in the unitary hypersphere of the strain space in the  of the parameter space of dimension 6 (corresponding a symmetric strain tensor in 3d).\cite{}.
%
From each trajectory, 40 snapshots are taken.
This ensures enough snapshots for our analysis.


From the training a series of displacement fluctuation, energy and damage snapshots
are obtained.
%
A following step will include the strain and energy bases generation, and reduced set of integration points for the RVE.
%
Elastic snapshost are processed separately guarantees an exact response during the elastic regime
%
Where each portion of the basis (ne elastic and ni inelastic modes) is
 obtained through a truncated Singular Value Decomposition (SVD) operation following the procedure described in \cite{} ???????
%
Validation set (or test set?) - Results are computed with cases randomly excluded from the training sets, and checking the the validation cases are clearly in no-linear regime.
%
\FloatBarrier
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Quantification of the approximation}
\label{sect_errors}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The accuracy of the solution obtained with the reduced order model is compared with the high fidelity computation for a particular validation trajectory, not included in the training set.
%
Using the bases and reduced integration points computed at the \emph{offline} stage.
%
Taking different combinations of strain modes and number of integration points.
%
For each combination, we compare the  difference of components of the homogenized stress tensor between the $\text{HRFE}^2$  ($\sigma_\text{HF}i$) and HF ($\sigma_\text{R}i$), and define the error as the maximum value (corresponding to the componente $i$) of the difference normalized by the norm of the homogenized stress tensor
%
\begin{equation}\label{eq_error}
\text{err} = \max \left(  \frac{ \| \sigma_\text{HF} i - \sigma_\text{R}i\| }{ \|\sigma_\text{HF}\|} \right)
\end{equation}
%
The obtained error curves for both RVE are shown  in figures \ref{fig_errors_ref} and \ref{fig_errors_porto}.
DEfine sigma HF, sigma R, component $i$


Comparison with ROM value (ROM esta definido?)
Convergence to ROM error with enough points taken.
All cases are well below the engineering \SI{1}{\percent}
%
\begin{figure}[hbt]
    \centering
    \includegraphics[width=\textwidth]{figures_results/fig_errors_ref_hf}
    \caption{Errors case reference. Dotted line ROM errors.}
    \label{fig_errors_ref}
\end{figure}
%
%
See Fig \ref{fig_errors_porto}.
%
\begin{figure}[hbt]
    \centering
    \includegraphics[width=\textwidth]{figures_results/fig_errors_porto_8r}
    \caption{Errors case Porto. Dotted line ROM errors. 70 modes overlaps 60 modes. }
    \label{fig_errors_porto}
\end{figure}
%
%
\FloatBarrier
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Model response}
\label{sect_response}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
reduced, it is still
driven by the original high-fidelity microscopic material models and
 therefore still obeys basic physical assumptions made at the microscale
(e.g. thermodynamic consistency, loading-unloading conditions).
%

- To test the obtained bases,, a homogeneous mesoscopic 1-element model (for hyper-reduction, this is actually a 1-element FE2 problem with a hyper-reduced micromodel)  with a single integration point and the same dimensions as the original micromodel is  used, with the fiber direction (1-axis) aligned with the mesoscopic x-axis. Macro strain $\sigma_\text{M} = $ [ \num{-0.076}, \num{0.748},
\num{0.188},
\num{0.539},
 \num{0.006},
 \num{-0.329}
].

Case Reference:
Curva con carga  y descarga, a pesar de no haber entrando la descarga. HF para comparar, pero fuera del training set. Error: \textcolor{red}{calcular}\%.
%
Reconstruction: See \ref{fig_reconstruction_ref} for qualitative comparison. Errors: Stress: \SI{1.87}{\percent}.  Damage: \SI{3.24}{\percent}.  Error between fields is computed as $\max (  \| \tilde{v}_i - v_i\|_1  /  \|v_i \|_1 )$.
%
\begin{figure}[hbt]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=0.99\textwidth]{figures_results/load_unload_ref}
        \caption{Load - unload cycle. Corresponding components of homogenized stress - strain curve. Untrained case. Training set trained only monotonically increasing strain. CASE REFERENCE}
    \end{subfigure}
    \begin{subfigure}[b]{0.55\textwidth}
        \includegraphics[height=3.0cm]{figures_results/damage_hf_ref}
        \includegraphics[height=3.0cm]{figures_results/damage_rve_ref}
        \includegraphics[height=3.0cm]{figures_results/damage_bar_ref}

        \includegraphics[height=3.0cm]{figures_results/stress_zz_hf_ref}
        \includegraphics[height=3.0cm]{figures_results/stress_zz_rve_ref}
        \includegraphics[height=3.0cm]{figures_results/stress_zz_bar_ref}
        \caption{Top: HF and reconstructed damage fields (\SI{3.24}{\percent} error). Bottom: stress zz fields (\SI{1.87}{\percent} error). Meshed deformed with fluctuant displacement. Values in cells are mean value of the value of its integration points.}
    \end{subfigure}
    \caption{Comparison HF - Reduced}
    \label{fig_reconstruction_ref}
\end{figure}
%
%

Case Porto:
Curva con carga  y descarga, a pesar de no haber entrando la descarga. HF para comparar, pero fuera del training set. Error: \textcolor{red}{calcular}\%.
%
Reconstruction: See \ref{fig_reconstruction_porto} for qualitative comparison. Errors: Stress: \SI{6.24}{\percent}.  Damage: \SI{6.20}{\percent} . Error between fields is computed as $\max (  \| \tilde{v}_i - v_i\|_1  /  \|v_i \|_1 )$.
%
\begin{figure}[hbt]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=0.99\textwidth]{figures_results/load_unload_porto.pdf}
        \caption{Load - unload cycle. Corresponding components of homogenized stress - strain curve. Untrained case. Training set trained only monotonically increasing strain. CASE PORTO. }
    \end{subfigure}
    \begin{subfigure}[b]{0.55\textwidth}
        \includegraphics[width=0.2\textwidth]{figures_results/damage_hf_porto}
        \includegraphics[width=0.3\textwidth]{figures_results/damage_rve_porto}
        \includegraphics[width=0.1\textwidth]{figures_results/damage_bar_porto}

        \includegraphics[width=0.2\textwidth]{figures_results/stress_hf_porto}
        \includegraphics[width=0.3\textwidth]{figures_results/stress_rve_porto}
        \includegraphics[width=0.1\textwidth]{figures_results/stress_bar_porto}

        \caption{
            \textcolor{red}{FALTA ACTUALIZAR FIGURAS HF}
             Main FEM (top) and reconstructed (bottom) fields.
            From left to right: stress XX, stress YY, damage, fluctuant displacement.
            Meshed deformed with fluctuant displacement.
            Values in cells are mean valor of the value of its integration points.
}
    \end{subfigure}
    \caption{Comparison HF - Reduced}
    \label{fig_reconstruction_porto}
\end{figure}
%
%
%
\FloatBarrier
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Customization}
\label{sect_customization}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The reduced RVE model employed in the previous sections is constructed in the bases of the material phase parameters depicted in.
In order to prove the tunability of the methodology in terms of the micromaterial phase parameters a number of customization tests are outlined, as seen in Tables \ref{tab:custom_params_ref} and \ref{tab:custom_params_porto}.
Comparison shown in figure~\ref{fig:custom_params}.
HRFE2 case 30m400ip.
Case not in the training dataset. Bases computed from dataset trained only in load part of the cycle.
Shows the resulting mechanical behaviour of the RVE obtained through a multiscale analysis and with a high fidelity analysis.
The multiscale analysis is based on the RVE reduced bases obtained from a sampling procedure based on the properties depicted in tables.
%
\begin{figure}[!hbt]
    \centering
    \includegraphics[width=0.49\textwidth]{figures_results/custom_material_ref}
    \includegraphics[width=0.49\textwidth]{figures_results/custom_material_porto}
    \caption{
        Stress - strain response for original material parameters and arbitrary customized material parameters as shown in table~\ref{tab:custom_params_ref} (model $A$, left), and table~\ref{tab:custom_params_porto} (model $B$, right).
    }
    \label{fig:custom_params}
\end{figure}
%
\begin{table}
    \centering
    \begin{tabular}{lc|cc}
        \toprule
                                                                                                                                                              &  Original   & Custom 1   &  Custom 2    \\
        \midrule
        Matrix: Young modulus E $[N/mm^2]$                                                                           & \num{3790}  &\textcolor{red}{\num{5000}} & \num{3790} \\
        Matrix: Poisson ratio $\nu$                                                                                                 & \num{0.37}    & \num{0.37}     &  \num{0.37} \\
        Matrix: Elastic threshold $\sigma_{\text{e}}$ $[N/mm^2]$                                    &  \num{200}    &  \textcolor{red}{\num{300}}     & \num{200} \\
        Matrix: Inf Elastic threshold $\sigma_{\text{e}}$ $[N/mm^2]$                             & \num{220}     & \textcolor{red}{\num{320}}     &  \num{220 } \\
        Matrix: Hardening parameter $H_1$                                                                             &  \num{0.10}   &\textcolor{red}{\num{0.5}} &   \num{0.10} \\
        Matrix: Hardening parameter $H_2$                                                                              & \num{0.01}    & \textcolor{red}{\num{0.1}} &  \num{0.01} \\
        \midrule
        Cohesive / Interply: Young modulus E $[N/mm^2]$                                                &  \num{3790}  & \num{3790}     & \num{ 3790} \\
        Cohesive / Interply: Poisson ratio $\nu$                                                                      &  \num{0.37}    &  \num{0.37}     & \num{ 0.37} \\
        Cohesive / Interply: Elastic threshold $\sigma_{\text{e}}$ $[N/mm^2]$         &  \num{100}     &  \num{100}      &  \num{100} \\
        Cohesive / Interply: Inf Elastic threshold $\sigma_{\text{e}}$ $[N/mm^2]$   &  \num{100.1} &  \num{100.1}   & \num{ 100.1} \\
        Cohesive / Interply: Hardening parameter $H_1$                                                     &  \num{0.01}    & \num{0.01}      &  \textcolor{red}{\num{0.9}} \\
        Cohesive / Interply: Hardening parameter $H_2$                                                    &  \num{0.01}   &  \num{0.01}      &  \textcolor{red}{\num{0.9 }} \\
        \bottomrule
    \end{tabular}
    \caption{Different modifications (colored text) to the material parameters of RVE matrix: \emph{Custom 1}: only modified the matrix values, interply material unchanged. \emph{Custom 2}: only modified interply material, matrix unchanged}
    \label{tab:custom_params_ref}
\end{table}
%
%
\begin{table}
    \centering
    \begin{tabular}{lc|ccc}
        \toprule
        &  Original   & Custom M1 & Custom M2 & Custom M3 \\
        \midrule
        Matrix: Young modulus E $[N/mm^2]$                                            & \num{4000}  &\textcolor{red}{\num{8000}} & \textcolor{red}{\num{8000}}  & \num{4000} \\
        Matrix: Poisson ratio $\nu$                                                                  & \num{0.38}    & \num{0.38}     &  \num{0.38} &  \num{0.38} \\
        Matrix: Elastic threshold $\sigma_{\text{e}}$ $[N/mm^2]$      &  \num{60}      &  \num{60}     & \num{60} & \num{60} \\
        Matrix: Inf Elastic threshold $\sigma_{\text{e}}$ $[N/mm^2]$& \num{70}       &  \num{70}     & \textcolor{red}{ \num{140}} &  \num{70} \\
        Matrix: Hardening parameter $H_1$                                                &  \num{0.335} &\num{0.335} &   \num{0.10}&   \num{0.335} \\
        Matrix: Hardening parameter $H_2$                                                & \num{0.05}     & \num{0.05} &  \num{0.01} &  \num{0.05} \\
        \midrule
        Inclusion: Young modulus E $[N/mm^2]$                                              &  \num{231000} & \num{231000}     &  \num{231000}    &  \num{231000}   \\
        Inclusion: Poisson ratio $\nu$                                                                    &  \num{0.2}         &  \num{0.2}             & \num{ 0.2}  & \num{0.2} \\
        Inclusion: Elastic threshold $\sigma_{\text{e}}$ $[N/mm^2]$        &  \num{1.0e8}    &  \num{1.0e8}         &   \num{1.0e8}   & \textcolor{red}{\num{60}} \\
        Inclusion: Inf Elastic threshold $\sigma_{\text{e}}$ $[N/mm^2]$  &  \num{1.1e8}   &  \num{1.1e8}          &   \num{1.1e8}   & \textcolor{red}{\num{70}} \\
        Inclusion: Hardening parameter $H_1$                                                   &  \num{0.01}     & \num{0.01}            &  \num{0.01} &  \num{0.01} \\
        Inclusion: Hardening parameter $H_2$                                                   &  \num{0.01}     &  \num{0.01}         &   \num{0.01}   &  \num{0.01}  \\
        \bottomrule
    \end{tabular}
    \caption{Different modifications (colored text) to the material parameters of RVE matrix: \emph{Custom 1}: only modified the matrix values, interply material unchanged. \emph{Custom 2}: only modified interply material, matrix unchanged}
    \label{tab:custom_params_porto}
\end{table}

\textcolor{red}{DESCRIBIR MODIFICACION DE MATERIALES. e.g. }First, the interphase hardening parameter and elastic limit is varied to the new values $H=0.1$ and $\sigma_{\text{e}}=175\:\text{MPa}$.
 If the material parameters are then modified the result is in good agreement  with the response obtained from a direct FE (high fidelity) computation using such user defined parameters.
 A more extreme customization case in which the hardening parameter of the matrix material is set to $H=0.9$ which is close to an elastic behaviour.
 It is then observed that 80 strain modes are required for the mutliscale analysis to correctly capture the desired behaviour.
 It is then concluded that a complete sampling renders a reduced basis capable of reproducing the mechanical behaviour upon changing the material phase parameters if enough strain modes are included in the reduced bases.
%
\FloatBarrier
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Computational and algorithmic Speed-up}
\label{sect_speedup}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The relative computational cost between standard $\text{FE}^2$ and the proposed $\text{RFE}^2$ technology is measured here through the algorithmic and computational speed-up, $S_p$. The algorithmic speed-up reflects the relative complexity of both techniques
in terms of the amount of DOF to solve (DOF speed-up) and amount of quadrature points (IP speed-up). Considering that an RVE basis with 40 strain modes and 200 quadrature points suffice to provide errors below $1\%$ when comparing the reduced order modelling and
high fidelity analysis, both DOF and IP speed-ups have been calculated considering 40 DOF and 200 IP in the reduced model. Figure~\ref{fig_speed-up} reflects the clearly growing algorithmic speed-ups upon
increasing the RVE discretization complexity. Based on the similar CRFC micro-structures with increasing number of layers and fibers one observes that for RVE discretizations with around one million of integration
points the relative algorithmic speed-up is around five orders of magnitude, i.e. the reduced RVE model is expected to perform $10^4$ times faster than the high fidelity one. Moreover, the reduced basis
inherits the type of boundary conditions utilized during the sampling stage and, therefore, avoids any performance overhead due to handling any multi-point constraints and their impact in the bandwidth of
the resulting system. Computation times have been compared regarding the high fidelity problem in one selected sampling trajectory and the reduced order model. It is seen that the resulting computational speed-up
increases even more upon increasing the RVE discretization and can reach around $30\times10^4$ for RVEs with around one million of integration points.
\begin{figure}
\centering
\includegraphics[width=0.8\textwidth]{figures_results/speedup}
\caption{\textcolor{red}{WIP FIGURE} Speedup en funcion de la precision, para diferentes tamaños de RVE}

\includegraphics[width=0.8\textwidth]{Figuras/fig_Speed-up}
\caption{Speed-up values upon increasing material discretization.}
\label{fig_speed-up}
\end{figure}
%
%
\FloatBarrier
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Multiscale reduced order modelling}
\label{sect_dogbone}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
A dogbone specimen as depicted in Figure~\ref{fig_dogbone} is considered in which an imposed displacement is applied at the basis around both extremes of the specimen.
The objective is to trigger, at the microstructural level, all delamination, fiber pull-out and debonding mechanisms.
%
\begin{figure}
    \centering
    \includegraphics[width=.7\textwidth]{figures_results/fig_dogbone}
    \caption{Multiscale analysis of a CRFC dogbone specimen under axial tension with shear: macroscopic geometry and boundary conditions.}
    \label{fig_dogbone}
\end{figure}
%
%
%\subsubsection{Case Reference}
%%
%Impact of the considered number of strain modes in the reduced RVE bases in the global response (see figure~\ref{fig:dogbone_reference_reaction}).
%%
%\begin{figure}
%    \centering
%    \includegraphics[width=0.8\textwidth]{figures_results/dogbone_reference_reaction}
%    \caption{Dogbone, 150 elems. RVE: Reference.  Nodal reaction. Comparison of the global mechanical response and error for different RVE. Reference values: 50 modes, 1600 ip}
%    \label{fig:dogbone_reference_reaction}
%\end{figure}
%%
%A deformed configuration of the dogbone together with a displacement reconstruction of an RVE (figure~\ref{fig:dogbone_reference_reconstruction_fields})
%%
%\begin{figure}
%    \centering
%    \includegraphics[height=5.0cm]{figures_results/macro_reaction_00_3}
%    \includegraphics[height=5.0cm]{figures_results/macro_reaction_00_1}
%    \includegraphics[height=5.0cm]{figures_results/macro_reaction_00_2}
%    \includegraphics[height=5.0cm]{figures_results/macro_reaction_00_bar}
%    \includegraphics[height=5.0cm]{figures_results/macro_stress_00_3}
%    \includegraphics[height=5.0cm]{figures_results/macro_stress_00_1}
%    \includegraphics[height=5.0cm]{figures_results/macro_stress_00_2}
%    \includegraphics[height=5.0cm]{figures_results/macro_stress_00_bar}
%    \includegraphics[width=0.45\textwidth]{figures_results/dogbone_rve_reconstruction_stress_porto_00}
%    \includegraphics[width=0.45\textwidth]{figures_results/dogbone_rve_reconstruction_damage_porto_00}
%    \caption{Deformed configuration of the macrostructure (top) and displacement reconstruction of an RVE corresponding to a critical stress point in the macro structure (bottom).}
%    \label{fig:dogbone_reference_reconstruction_fields}
%\end{figure}
%
%
\subsubsection{Case Porto (longitudinal fibres)}
%
Impact of the considered number of strain modes in the reduced RVE bases in the global response (see figure~\ref{fig:dogbone_reaction_porto_parallel}).
%
\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{figures_results/dogbone_reaction_porto_long}
    \caption{Multiscale: dogbone 150 elems. RVE porto (longitudinal). Nodal reaction. Comparison of global mechanical response using different strain modes and points. Reference: 50m1800ip.}
    \label{fig:dogbone_reaction_porto_long}
\end{figure}
%
A deformed configuration of the dogbone together with a displacement reconstruction of an RVE (figure~\ref{fig:dogbone_porto_reconstruction_fields_long})
%
\begin{figure}
    \centering
    %\includegraphics[width=0.25\textwidth]{figures_results/macro_reaction_90_3}
    %\includegraphics[width=0.25\textwidth]{figures_results/macro_reaction_90_1}
    %\includegraphics[width=0.25\textwidth]{figures_results/macro_reaction_90_2}
    %\includegraphics[width=0.08\textwidth]{figures_results/macro_reaction_90_bar}
    \includegraphics[width=0.25\textwidth]{figures_results/macro_stress_90_3}
    \includegraphics[width=0.25\textwidth]{figures_results/macro_stress_90_1}
    \includegraphics[width=0.25\textwidth]{figures_results/macro_stress_90_2}
    \includegraphics[width=0.08\textwidth]{figures_results/macro_stress_90_bar}
    \includegraphics[width=0.45\textwidth]{figures_results/dogbone_rve_reconstruction_stress_porto_90}
    \includegraphics[width=0.45\textwidth]{figures_results/dogbone_rve_reconstruction_damage_porto_90}    \includegraphics[width=0.45\textwidth]{figures_results/dogbone_rve_reconstruction_stress_porto_long_2}
    \includegraphics[width=0.45\textwidth]{figures_results/dogbone_rve_reconstruction_damage_porto_long_2}
    \caption{Deformed configuration of the macrostructure (top) and displacement reconstruction of an RVE.}
    \label{fig:dogbone_porto_reconstruction_fields_long}
\end{figure}
%
Customized material with original bases. \textcolor{red}{Reference with bases computed for the new material}, for quantification of error (see figure~\ref{fig:dogbone_porto_reaction_custom_long}).
%
\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{figures_results/dogbone_reaction_custom_porto_long}
    \caption{\textcolor{red}{Referencia es 50-1800-REAL, pero se muestra 20-100-REAL de momento.} Multiscale: dogbone 150 elems. RVE porto (longitudinal). Nodal reaction. Mechanical response using parameter materials different from the original in the bases. Reference value is obtained from bases  computd with modified materials.}
    \label{fig:dogbone_porto_reaction_custom_long}
\end{figure}
%
%
\FloatBarrier
\subsubsection{Case Porto (transverse fibres)}
%
Impact of the considered number of strain modes in the reduced RVE bases in the global response (see figure~\ref{fig:dogbone_reaction_porto_trans}).
%
\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{figures_results/dogbone_reaction_porto_00}
    \caption{Multiscale: dogbone 150 elems. RVE porto (transverse). Nodal reaction. Comparison of global mechanical response using different strain modes and points.}
    \label{fig:dogbone_reaction_porto_trans}
\end{figure}
%
A deformed configuration of the dogbone together with a displacement reconstruction of an RVE (figure~\ref{fig:dogbone_porto_reconstruction_fields_trans})
%
\begin{figure}
    \centering
    \includegraphics[height=5.0cm]{figures_results/macro_reaction_00_3}
    \includegraphics[height=5.0cm]{figures_results/macro_reaction_00_1}
    \includegraphics[height=5.0cm]{figures_results/macro_reaction_00_2}
    \includegraphics[height=5.0cm]{figures_results/macro_reaction_00_bar}
    \includegraphics[height=5.0cm]{figures_results/macro_stress_00_3}
    \includegraphics[height=5.0cm]{figures_results/macro_stress_00_1}
    \includegraphics[height=5.0cm]{figures_results/macro_stress_00_2}
    \includegraphics[height=5.0cm]{figures_results/macro_stress_00_bar}
    \includegraphics[width=0.45\textwidth]{figures_results/dogbone_rve_reconstruction_stress_porto_00}
    \includegraphics[width=0.45\textwidth]{figures_results/dogbone_rve_reconstruction_damage_porto_00}
    \caption{Deformed configuration of the macrostructure (top) and displacement reconstruction of an RVE corresponding to a critical stress point in the macro structure (bottom).}
    \label{fig:dogbone_porto_reconstruction_fields_trans}
\end{figure}
%
Customized material with original bases. Reference with bases computed for the new material, for quantification of error (see figure~\ref{fig:dogbone_porto_reaction_custom_trans}).
%
\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{figures_results/dogbone_reaction_custom_porto_perpendicular}
    \caption{DOGBONE (Perpendicular). 150 elems. RVE: Reference.  Average reaction. Global mechanical response upon increasing the micro strain modes.}
    \label{fig:dogbone_porto_reaction_custom_trans}
\end{figure}
\FloatBarrier
